Exploiting Intraday Decompositions in Realized Volatility Forecasting: A Forecast Reconciliation Approach

We address the construction of Realized Variance (RV) forecasts by exploiting the hierarchical structure implicit in available decompositions of RV. By using data referred to the Dow Jones Industrial Average Index and to its constituents we show that exploiting the informative content of hierarchies improves the forecast accuracy. Forecasting performance is evaluated out-of-sample based on the empirical MSE and QLIKE criteria as well as using the Model Confidence Set approach.

==> tab/geomean/geomean_all_11.tex <==

\begin{tabular}[t]{>{}c|cc>{}c|ccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} \\
 & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{c}{\textit{Panel A: DJIA index}}\\
$SV$ & \textcolor{red}{1.028} & \textcolor{red}{1.017} & \textcolor{red}{1.003} & \textcolor{black}{0.973} & \textcolor{black}{0.997} & \textcolor{black}{0.928}\\
$SV_{bu}$ & \textcolor{black}{0.960} & \textcolor{black}{0.972} & \textcolor{red}{1.005} & \textcolor{red}{1.010} & \textcolor{black}{0.237} & \textcolor{black}{0.748}\\
$TSV_{bu}$ & \textcolor{black}{0.824} & \textcolor{black}{0.801} & \textcolor{red}{1.099} & \textcolor{red}{1.085} & \textcolor{black}{0.249} & \textcolor{black}{0.385}\\
$SV_{shr}$ & \textcolor{black}{0.976} & \textcolor{black}{0.991} & \textcolor{red}{1.002} & \textcolor{black}{0.983} & \textcolor{black}{0.233} & \textcolor{black}{0.728}\\
$TSV_{shr}$ & \textcolor{black}{0.869} & \textcolor{black}{0.878} & \textcolor{black}{0.965} & \textcolor{red}{1.011} & \textcolor{black}{0.236} & \textcolor{black}{0.379}\\
$PV(3)$ & \textcolor{black}{0.816} & \textcolor{red}{1.077} & \textcolor{red}{1.025} & \textcolor{red}{2.272} & \textcolor{black}{0.977} & \textcolor{black}{0.962}\\
$PV(3)_{bu}$ & \textcolor{black}{0.924} & \textcolor{black}{0.957} & \textcolor{red}{1.009} & \textcolor{red}{1.001} & \textcolor{black}{0.235} & \textcolor{black}{0.596}\\
$TPV(3)_{bu}$ & \textcolor{black}{0.822} & \textcolor{black}{\textbf{0.795}} & \textcolor{red}{1.103} & \textcolor{red}{1.090} & \textcolor{black}{0.250} & \textcolor{black}{0.386}\\
$PV(3)_{shr}$ & \textcolor{black}{0.833} & \textcolor{red}{1.015} & \textcolor{red}{1.015} & \textcolor{black}{\textbf{0.945}} & \textcolor{black}{\textbf{0.225}} & \textcolor{black}{0.596}\\
$TPV(3)_{shr}$ & \textcolor{black}{\textbf{0.808}} & \textcolor{black}{0.925} & \textcolor{black}{\textbf{0.939}} & \textcolor{black}{0.971} & \textcolor{black}{0.227} & \textcolor{black}{\textbf{0.374}}\\
\addlinespace[0.3em]
\multicolumn{7}{c}{\textit{Panel B: Individual stocks}}\\
$SV$ & \textcolor{red}{1.016} & \textcolor{red}{1.008} & \textcolor{red}{1.001} & \textcolor{red}{1.092} & \textcolor{black}{0.998} & \textcolor{black}{0.993}\\
$SV_{bu}$ & \textcolor{black}{0.964} & \textcolor{black}{0.992} & \textcolor{black}{0.998} & \textcolor{black}{0.921} & \textcolor{black}{0.977} & \textcolor{black}{0.971}\\
$TSV_{bu}$ & \textcolor{black}{0.991} & \textcolor{red}{1.054} & \textcolor{red}{1.019} & \textcolor{black}{0.893} & \textcolor{black}{0.908} & \textcolor{black}{0.875}\\
$SV_{shr}$ & \textcolor{black}{0.980} & \textcolor{black}{0.996} & \textcolor{black}{0.998} & \textcolor{black}{0.899} & \textcolor{black}{0.947} & \textcolor{black}{0.960}\\
$TSV_{shr}$ & \textcolor{black}{0.987} & \textcolor{red}{1.007} & \textcolor{black}{0.984} & \textcolor{black}{0.850} & \textcolor{black}{0.861} & \textcolor{black}{0.853}\\
$PV(3)$ & \textcolor{black}{0.899} & \textcolor{black}{0.976} & \textcolor{red}{1.010} & \textcolor{red}{1.364} & \textcolor{red}{1.025} & \textcolor{red}{1.055}\\
$PV(3)_{bu}$ & \textcolor{black}{0.943} & \textcolor{black}{0.982} & \textcolor{black}{0.995} & \textcolor{black}{0.900} & \textcolor{black}{0.895} & \textcolor{black}{0.945}\\
$TPV(3)_{bu}$ & \textcolor{black}{0.982} & \textcolor{red}{1.039} & \textcolor{red}{1.012} & \textcolor{black}{0.894} & \textcolor{black}{0.902} & \textcolor{black}{0.868}\\
$PV(3)_{shr}$ & \textcolor{black}{\textbf{0.896}} & \textcolor{black}{\textbf{0.964}} & \textcolor{black}{0.994} & \textcolor{black}{0.833} & \textcolor{black}{0.824} & \textcolor{black}{0.916}\\
$TPV(3)_{shr}$ & \textcolor{black}{0.924} & \textcolor{black}{0.967} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{\textbf{0.805}} & \textcolor{black}{\textbf{0.793}} & \textcolor{black}{\textbf{0.824}}\\
\bottomrule
\end{tabular}


==> tab/geomean/geomean_groups_11.tex <==

\begin{tabular}[t]{>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|ccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{2007-2010} & \multicolumn{6}{c}{2011-2014} & \multicolumn{6}{c}{2015-2019} & \multicolumn{6}{c}{2020-2022} \\
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} \\
 & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$\\
\midrule
\addlinespace[0.3em]
\multicolumn{25}{c}{\textit{Panel A: DJIA index}}\\
$SV$ & \textcolor{red}{1.024} & \textcolor{red}{1.012} & \textcolor{red}{1.002} & \textcolor{black}{0.978} & \textcolor{black}{0.985} & \textcolor{red}{1.001} & \textcolor{black}{0.991} & \textcolor{red}{1.011} & \textcolor{black}{\textbf{0.998}} & \textcolor{black}{\textbf{0.986}} & \textcolor{black}{\textbf{0.988}} & \textcolor{black}{\textbf{0.999}} & \textcolor{red}{1.069} & \textcolor{black}{0.999} & \textcolor{red}{1.003} & \textcolor{black}{0.968} & \textcolor{black}{0.986} & \textcolor{black}{0.996} & \textcolor{red}{1.048} & \textcolor{red}{1.030} & \textcolor{red}{1.006} & \textcolor{black}{0.962} & \textcolor{black}{1.000} & \textcolor{black}{0.904}\\
$SV_{bu}$ & \textcolor{black}{0.962} & \textcolor{black}{0.991} & \textcolor{red}{1.007} & \textcolor{red}{1.024} & \textcolor{red}{1.014} & \textcolor{red}{1.011} & \textcolor{red}{1.055} & \textcolor{red}{1.016} & \textcolor{red}{1.007} & \textcolor{red}{1.069} & \textcolor{red}{1.049} & \textcolor{red}{1.014} & \textcolor{black}{0.966} & \textcolor{black}{0.985} & \textcolor{black}{0.991} & \textcolor{red}{1.021} & \textcolor{red}{1.021} & \textcolor{red}{1.004} & \textcolor{black}{0.923} & \textcolor{black}{0.921} & \textcolor{red}{\textbf{1.003}} & \textcolor{black}{0.897} & \textcolor{black}{0.051} & \textcolor{black}{0.662}\\
$TSV_{bu}$ & \textcolor{black}{0.801} & \textcolor{black}{0.774} & \textcolor{red}{1.121} & \textcolor{red}{1.085} & \textcolor{red}{1.063} & \textcolor{red}{1.047} & \textcolor{red}{1.151} & \textcolor{red}{1.072} & \textcolor{red}{1.055} & \textcolor{red}{1.245} & \textcolor{red}{1.210} & \textcolor{red}{1.092} & \textcolor{black}{0.914} & \textcolor{black}{0.977} & \textcolor{black}{0.991} & \textcolor{red}{1.074} & \textcolor{red}{1.045} & \textcolor{red}{1.006} & \textcolor{black}{0.923} & \textcolor{black}{0.833} & \textcolor{red}{1.035} & \textcolor{black}{0.906} & \textcolor{black}{0.051} & \textcolor{black}{0.170}\\
$SV_{shr}$ & \textcolor{black}{0.976} & \textcolor{black}{0.998} & \textcolor{red}{1.002} & \textcolor{black}{0.997} & \textcolor{black}{0.995} & \textcolor{red}{1.006} & \textcolor{red}{1.022} & \textcolor{red}{1.006} & \textcolor{red}{1.003} & \textcolor{red}{1.027} & \textcolor{red}{1.020} & \textcolor{red}{1.007} & \textcolor{black}{0.997} & \textcolor{black}{0.983} & \textcolor{black}{1.000} & \textcolor{black}{0.989} & \textcolor{black}{0.995} & \textcolor{black}{0.996} & \textcolor{black}{0.960} & \textcolor{black}{0.975} & \textcolor{red}{1.003} & \textcolor{black}{0.896} & \textcolor{black}{0.053} & \textcolor{black}{0.637}\\
$TSV_{shr}$ & \textcolor{black}{0.856} & \textcolor{black}{0.853} & \textcolor{black}{0.949} & \textcolor{red}{1.020} & \textcolor{red}{1.009} & \textcolor{red}{1.014} & \textcolor{red}{1.066} & \textcolor{red}{1.031} & \textcolor{red}{1.044} & \textcolor{red}{1.109} & \textcolor{red}{1.094} & \textcolor{red}{1.053} & \textcolor{black}{0.930} & \textcolor{black}{0.967} & \textcolor{red}{1.005} & \textcolor{red}{1.011} & \textcolor{black}{0.999} & \textcolor{black}{0.997} & \textcolor{black}{0.923} & \textcolor{black}{0.920} & \textcolor{red}{1.010} & \textcolor{black}{\textbf{0.873}} & \textcolor{black}{0.050} & \textcolor{black}{\textbf{0.169}}\\
$PV(3)$ & \textcolor{black}{\textbf{0.775}} & \textcolor{red}{1.047} & \textcolor{red}{1.030} & \textcolor{red}{2.691} & \textcolor{red}{1.645} & \textcolor{black}{\textbf{0.995}} & \textcolor{black}{\textbf{0.921}} & \textcolor{black}{0.973} & \textcolor{red}{1.001} & \textcolor{red}{1.073} & \textcolor{red}{1.021} & \textcolor{red}{1.011} & \textcolor{black}{0.997} & \textcolor{red}{1.013} & \textcolor{black}{0.988} & \textcolor{black}{\textbf{0.873}} & \textcolor{black}{\textbf{0.908}} & \textcolor{black}{\textbf{0.969}} & \textcolor{red}{1.059} & \textcolor{red}{1.163} & \textcolor{red}{1.012} & \textcolor{red}{6.045} & \textcolor{black}{0.942} & \textcolor{black}{0.954}\\
$PV(3)_{bu}$ & \textcolor{black}{0.922} & \textcolor{black}{0.981} & \textcolor{red}{1.010} & \textcolor{red}{1.023} & \textcolor{red}{1.015} & \textcolor{red}{1.011} & \textcolor{red}{1.036} & \textcolor{red}{1.013} & \textcolor{red}{1.009} & \textcolor{red}{1.076} & \textcolor{red}{1.058} & \textcolor{red}{1.021} & \textcolor{black}{0.947} & \textcolor{black}{0.979} & \textcolor{black}{0.988} & \textcolor{red}{1.004} & \textcolor{red}{1.011} & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.911}} & \textcolor{black}{0.892} & \textcolor{red}{1.006} & \textcolor{black}{0.874} & \textcolor{black}{\textbf{0.049}} & \textcolor{black}{0.460}\\
$TPV(3)_{bu}$ & \textcolor{black}{0.799} & \textcolor{black}{\textbf{0.766}} & \textcolor{red}{1.125} & \textcolor{red}{1.092} & \textcolor{red}{1.067} & \textcolor{red}{1.054} & \textcolor{red}{1.148} & \textcolor{red}{1.078} & \textcolor{red}{1.064} & \textcolor{red}{1.265} & \textcolor{red}{1.231} & \textcolor{red}{1.106} & \textcolor{black}{0.911} & \textcolor{black}{0.978} & \textcolor{black}{0.991} & \textcolor{red}{1.075} & \textcolor{red}{1.049} & \textcolor{red}{1.007} & \textcolor{black}{0.916} & \textcolor{black}{\textbf{0.832}} & \textcolor{red}{1.037} & \textcolor{black}{0.893} & \textcolor{black}{0.051} & \textcolor{black}{0.169}\\
$PV(3)_{shr}$ & \textcolor{black}{0.812} & \textcolor{red}{1.010} & \textcolor{red}{1.018} & \textcolor{black}{\textbf{0.941}} & \textcolor{black}{\textbf{0.946}} & \textcolor{red}{1.000} & \textcolor{black}{0.944} & \textcolor{black}{\textbf{0.963}} & \textcolor{red}{1.003} & \textcolor{red}{1.047} & \textcolor{red}{1.030} & \textcolor{red}{1.015} & \textcolor{black}{0.934} & \textcolor{black}{0.975} & \textcolor{black}{\textbf{0.983}} & \textcolor{black}{0.902} & \textcolor{black}{0.938} & \textcolor{black}{0.976} & \textcolor{black}{0.947} & \textcolor{red}{1.033} & \textcolor{red}{1.005} & \textcolor{black}{0.902} & \textcolor{black}{0.051} & \textcolor{black}{0.465}\\
$TPV(3)_{shr}$ & \textcolor{black}{0.787} & \textcolor{black}{0.909} & \textcolor{black}{\textbf{0.914}} & \textcolor{black}{0.967} & \textcolor{black}{0.956} & \textcolor{black}{0.997} & \textcolor{black}{0.992} & \textcolor{black}{0.984} & \textcolor{red}{1.057} & \textcolor{red}{1.095} & \textcolor{red}{1.061} & \textcolor{red}{1.032} & \textcolor{black}{\textbf{0.900}} & \textcolor{black}{\textbf{0.962}} & \textcolor{black}{0.989} & \textcolor{black}{0.944} & \textcolor{black}{0.948} & \textcolor{black}{0.977} & \textcolor{black}{0.915} & \textcolor{black}{0.956} & \textcolor{red}{1.012} & \textcolor{black}{0.874} & \textcolor{black}{0.050} & \textcolor{black}{0.169}\\
\addlinespace[0.3em]
\multicolumn{25}{c}{\textit{Panel B: Individual stocks}}\\
$SV$ & \textcolor{black}{0.993} & \textcolor{red}{1.014} & \textcolor{red}{1.001} & \textcolor{red}{1.124} & \textcolor{red}{1.004} & \textcolor{black}{1.000} & \textcolor{red}{1.022} & \textcolor{black}{0.985} & \textcolor{black}{0.990} & \textcolor{red}{1.076} & \textcolor{black}{0.982} & \textcolor{black}{0.988} & \textcolor{red}{1.005} & \textcolor{red}{1.001} & \textcolor{red}{1.005} & \textcolor{red}{1.080} & \textcolor{black}{0.993} & \textcolor{black}{0.997} & \textcolor{red}{1.073} & \textcolor{red}{1.005} & \textcolor{red}{1.001} & \textcolor{black}{0.963} & \textcolor{red}{1.025} & \textcolor{black}{0.994}\\
$SV_{bu}$ & \textcolor{black}{0.967} & \textcolor{black}{0.991} & \textcolor{black}{0.998} & \textcolor{red}{1.000} & \textcolor{red}{1.010} & \textcolor{red}{1.008} & \textcolor{red}{1.000} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.007} & \textcolor{red}{1.008} & \textcolor{red}{1.003} & \textcolor{black}{0.973} & \textcolor{black}{0.991} & \textcolor{black}{0.992} & \textcolor{red}{1.006} & \textcolor{black}{0.999} & \textcolor{black}{0.995} & \textcolor{black}{0.998} & \textcolor{red}{1.000} & \textcolor{red}{1.001} & \textcolor{black}{0.779} & \textcolor{black}{0.946} & \textcolor{black}{0.942}\\
$TSV_{bu}$ & \textcolor{red}{1.028} & \textcolor{red}{1.004} & \textcolor{red}{1.043} & \textcolor{red}{1.019} & \textcolor{red}{1.076} & \textcolor{red}{1.051} & \textcolor{red}{1.060} & \textcolor{red}{1.048} & \textcolor{red}{1.043} & \textcolor{red}{1.119} & \textcolor{red}{1.108} & \textcolor{red}{1.055} & \textcolor{black}{0.867} & \textcolor{black}{0.994} & \textcolor{black}{0.960} & \textcolor{red}{1.029} & \textcolor{black}{0.994} & \textcolor{black}{0.980} & \textcolor{red}{1.023} & \textcolor{red}{1.021} & \textcolor{red}{1.006} & \textcolor{black}{0.656} & \textcolor{black}{0.698} & \textcolor{black}{0.730}\\
$SV_{shr}$ & \textcolor{black}{0.970} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.992} & \textcolor{red}{1.001} & \textcolor{red}{1.003} & \textcolor{black}{0.985} & \textcolor{black}{0.987} & \textcolor{black}{0.993} & \textcolor{black}{0.988} & \textcolor{black}{0.991} & \textcolor{black}{0.995} & \textcolor{black}{0.979} & \textcolor{black}{0.992} & \textcolor{black}{0.995} & \textcolor{black}{0.987} & \textcolor{black}{0.990} & \textcolor{black}{0.993} & \textcolor{red}{1.029} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{black}{0.742} & \textcolor{black}{0.897} & \textcolor{black}{0.927}\\
$TSV_{shr}$ & \textcolor{red}{1.009} & \textcolor{black}{0.987} & \textcolor{black}{0.994} & \textcolor{black}{0.959} & \textcolor{red}{1.018} & \textcolor{red}{1.016} & \textcolor{red}{1.014} & \textcolor{red}{1.010} & \textcolor{red}{1.018} & \textcolor{red}{1.041} & \textcolor{red}{1.043} & \textcolor{red}{1.023} & \textcolor{black}{0.907} & \textcolor{black}{0.987} & \textcolor{black}{0.971} & \textcolor{black}{0.991} & \textcolor{black}{0.979} & \textcolor{black}{0.979} & \textcolor{black}{0.997} & \textcolor{black}{0.988} & \textcolor{black}{0.990} & \textcolor{black}{0.632} & \textcolor{black}{0.646} & \textcolor{black}{0.706}\\
$PV(3)$ & \textcolor{black}{0.938} & \textcolor{red}{1.035} & \textcolor{red}{1.049} & \textcolor{red}{1.421} & \textcolor{red}{1.139} & \textcolor{black}{\textbf{0.980}} & \textcolor{black}{0.973} & \textcolor{black}{0.958} & \textcolor{black}{\textbf{0.990}} & \textcolor{red}{1.046} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.976}} & \textcolor{black}{\textbf{0.836}} & \textcolor{black}{\textbf{0.943}} & \textcolor{black}{\textbf{0.941}} & \textcolor{red}{1.344} & \textcolor{red}{1.029} & \textcolor{red}{1.016} & \textcolor{red}{1.097} & \textcolor{black}{0.978} & \textcolor{black}{0.964} & \textcolor{red}{1.035} & \textcolor{black}{0.865} & \textcolor{red}{1.106}\\
$PV(3)_{bu}$ & \textcolor{black}{0.953} & \textcolor{black}{0.981} & \textcolor{black}{0.997} & \textcolor{red}{1.003} & \textcolor{red}{1.010} & \textcolor{red}{1.009} & \textcolor{black}{0.993} & \textcolor{black}{0.999} & \textcolor{red}{1.004} & \textcolor{red}{1.010} & \textcolor{red}{1.013} & \textcolor{red}{1.008} & \textcolor{black}{0.950} & \textcolor{black}{0.984} & \textcolor{black}{0.980} & \textcolor{black}{0.990} & \textcolor{black}{0.984} & \textcolor{black}{0.982} & \textcolor{black}{0.994} & \textcolor{black}{0.990} & \textcolor{black}{0.997} & \textcolor{black}{0.709} & \textcolor{black}{0.750} & \textcolor{black}{0.899}\\
$TPV(3)_{bu}$ & \textcolor{red}{1.027} & \textcolor{black}{0.996} & \textcolor{red}{1.038} & \textcolor{red}{1.029} & \textcolor{red}{1.083} & \textcolor{red}{1.058} & \textcolor{red}{1.063} & \textcolor{red}{1.055} & \textcolor{red}{1.053} & \textcolor{red}{1.134} & \textcolor{red}{1.123} & \textcolor{red}{1.065} & \textcolor{black}{0.859} & \textcolor{black}{0.994} & \textcolor{black}{0.955} & \textcolor{red}{1.030} & \textcolor{black}{0.993} & \textcolor{black}{0.978} & \textcolor{red}{1.011} & \textcolor{red}{1.000} & \textcolor{black}{1.000} & \textcolor{black}{0.641} & \textcolor{black}{0.655} & \textcolor{black}{0.712}\\
$PV(3)_{shr}$ & \textcolor{black}{\textbf{0.916}} & \textcolor{black}{0.998} & \textcolor{red}{1.017} & \textcolor{black}{0.939} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{0.983} & \textcolor{black}{\textbf{0.927}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{0.993} & \textcolor{black}{\textbf{0.970}} & \textcolor{black}{0.965} & \textcolor{black}{0.988} & \textcolor{black}{0.874} & \textcolor{black}{0.949} & \textcolor{black}{0.949} & \textcolor{black}{\textbf{0.898}} & \textcolor{black}{0.929} & \textcolor{black}{0.961} & \textcolor{red}{1.030} & \textcolor{black}{0.971} & \textcolor{black}{0.970} & \textcolor{black}{0.704} & \textcolor{black}{0.662} & \textcolor{black}{0.865}\\
$TPV(3)_{shr}$ & \textcolor{black}{0.963} & \textcolor{black}{\textbf{0.973}} & \textcolor{black}{\textbf{0.982}} & \textcolor{black}{\textbf{0.923}} & \textcolor{black}{0.963} & \textcolor{black}{0.989} & \textcolor{black}{0.963} & \textcolor{black}{0.972} & \textcolor{red}{1.013} & \textcolor{red}{1.013} & \textcolor{black}{0.990} & \textcolor{black}{0.996} & \textcolor{black}{0.848} & \textcolor{black}{0.955} & \textcolor{black}{0.941} & \textcolor{black}{0.918} & \textcolor{black}{\textbf{0.924}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.991}} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{\textbf{0.606}} & \textcolor{black}{\textbf{0.565}} & \textcolor{black}{\textbf{0.672}}\\
\bottomrule
\end{tabular}


==> tab/geomean/geomean_groups_5.tex <==

\begin{tabular}[t]{>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|ccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{2007-2010} & \multicolumn{6}{c}{2011-2014} & \multicolumn{6}{c}{2015-2019} & \multicolumn{6}{c}{2020-2022} \\
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} \\
 & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$\\
\midrule
\addlinespace[0.3em]
\multicolumn{25}{c}{\textit{Panel A: DJIA index}}\\
$TSV_{bu}$ & \textcolor{black}{0.801} & \textcolor{black}{0.774} & \textcolor{red}{1.121} & \textcolor{red}{1.085} & \textcolor{red}{1.063} & \textcolor{red}{1.047} & \textcolor{red}{1.151} & \textcolor{red}{1.072} & \textcolor{red}{1.055} & \textcolor{red}{1.245} & \textcolor{red}{1.210} & \textcolor{red}{1.092} & \textcolor{black}{0.914} & \textcolor{black}{0.977} & \textcolor{black}{0.991} & \textcolor{red}{1.074} & \textcolor{red}{1.045} & \textcolor{red}{1.006} & \textcolor{black}{0.923} & \textcolor{black}{0.833} & \textcolor{red}{1.035} & \textcolor{black}{0.906} & \textcolor{black}{0.051} & \textcolor{black}{0.170}\\
$TSV_{shr}$ & \textcolor{black}{0.856} & \textcolor{black}{0.853} & \textcolor{black}{0.949} & \textcolor{red}{1.020} & \textcolor{red}{1.009} & \textcolor{red}{1.014} & \textcolor{red}{1.066} & \textcolor{red}{1.031} & \textcolor{red}{\textbf{1.044}} & \textcolor{red}{1.109} & \textcolor{red}{1.094} & \textcolor{red}{1.053} & \textcolor{black}{0.930} & \textcolor{black}{0.967} & \textcolor{red}{1.005} & \textcolor{red}{1.011} & \textcolor{black}{0.999} & \textcolor{black}{0.997} & \textcolor{black}{0.923} & \textcolor{black}{0.920} & \textcolor{red}{\textbf{1.010}} & \textcolor{black}{\textbf{0.873}} & \textcolor{black}{0.050} & \textcolor{black}{\textbf{0.169}}\\
$TPV(3)_{bu}$ & \textcolor{black}{0.799} & \textcolor{black}{\textbf{0.766}} & \textcolor{red}{1.125} & \textcolor{red}{1.092} & \textcolor{red}{1.067} & \textcolor{red}{1.054} & \textcolor{red}{1.148} & \textcolor{red}{1.078} & \textcolor{red}{1.064} & \textcolor{red}{1.265} & \textcolor{red}{1.231} & \textcolor{red}{1.106} & \textcolor{black}{0.911} & \textcolor{black}{0.978} & \textcolor{black}{0.991} & \textcolor{red}{1.075} & \textcolor{red}{1.049} & \textcolor{red}{1.007} & \textcolor{black}{0.916} & \textcolor{black}{\textbf{0.832}} & \textcolor{red}{1.037} & \textcolor{black}{0.893} & \textcolor{black}{0.051} & \textcolor{black}{0.169}\\
$TPV(3)_{shr}$ & \textcolor{black}{\textbf{0.787}} & \textcolor{black}{0.909} & \textcolor{black}{\textbf{0.914}} & \textcolor{black}{\textbf{0.967}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.997}} & \textcolor{black}{\textbf{0.992}} & \textcolor{black}{\textbf{0.984}} & \textcolor{red}{1.057} & \textcolor{red}{\textbf{1.095}} & \textcolor{red}{\textbf{1.061}} & \textcolor{red}{\textbf{1.032}} & \textcolor{black}{\textbf{0.900}} & \textcolor{black}{\textbf{0.962}} & \textcolor{black}{\textbf{0.989}} & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.948}} & \textcolor{black}{\textbf{0.977}} & \textcolor{black}{\textbf{0.915}} & \textcolor{black}{0.956} & \textcolor{red}{1.012} & \textcolor{black}{0.874} & \textcolor{black}{\textbf{0.050}} & \textcolor{black}{0.169}\\
\addlinespace[0.3em]
\multicolumn{25}{c}{\textit{Panel B: Individual stocks}}\\
$TSV_{bu}$ & \textcolor{red}{1.028} & \textcolor{red}{1.004} & \textcolor{red}{1.043} & \textcolor{red}{1.019} & \textcolor{red}{1.076} & \textcolor{red}{1.051} & \textcolor{red}{1.060} & \textcolor{red}{1.048} & \textcolor{red}{1.043} & \textcolor{red}{1.119} & \textcolor{red}{1.108} & \textcolor{red}{1.055} & \textcolor{black}{0.867} & \textcolor{black}{0.994} & \textcolor{black}{0.960} & \textcolor{red}{1.029} & \textcolor{black}{0.994} & \textcolor{black}{0.980} & \textcolor{red}{1.023} & \textcolor{red}{1.021} & \textcolor{red}{1.006} & \textcolor{black}{0.656} & \textcolor{black}{0.698} & \textcolor{black}{0.730}\\
$TSV_{shr}$ & \textcolor{red}{1.009} & \textcolor{black}{0.987} & \textcolor{black}{0.994} & \textcolor{black}{0.959} & \textcolor{red}{1.018} & \textcolor{red}{1.016} & \textcolor{red}{1.014} & \textcolor{red}{1.010} & \textcolor{red}{1.018} & \textcolor{red}{1.041} & \textcolor{red}{1.043} & \textcolor{red}{1.023} & \textcolor{black}{0.907} & \textcolor{black}{0.987} & \textcolor{black}{0.971} & \textcolor{black}{0.991} & \textcolor{black}{0.979} & \textcolor{black}{0.979} & \textcolor{black}{0.997} & \textcolor{black}{0.988} & \textcolor{black}{0.990} & \textcolor{black}{0.632} & \textcolor{black}{0.646} & \textcolor{black}{0.706}\\
$TPV(3)_{bu}$ & \textcolor{red}{1.027} & \textcolor{black}{0.996} & \textcolor{red}{1.038} & \textcolor{red}{1.029} & \textcolor{red}{1.083} & \textcolor{red}{1.058} & \textcolor{red}{1.063} & \textcolor{red}{1.055} & \textcolor{red}{1.053} & \textcolor{red}{1.134} & \textcolor{red}{1.123} & \textcolor{red}{1.065} & \textcolor{black}{0.859} & \textcolor{black}{0.994} & \textcolor{black}{0.955} & \textcolor{red}{1.030} & \textcolor{black}{0.993} & \textcolor{black}{0.978} & \textcolor{red}{1.011} & \textcolor{red}{1.000} & \textcolor{black}{1.000} & \textcolor{black}{0.641} & \textcolor{black}{0.655} & \textcolor{black}{0.712}\\
$TPV(3)_{shr}$ & \textcolor{black}{\textbf{0.963}} & \textcolor{black}{\textbf{0.973}} & \textcolor{black}{\textbf{0.982}} & \textcolor{black}{\textbf{0.923}} & \textcolor{black}{\textbf{0.963}} & \textcolor{black}{\textbf{0.989}} & \textcolor{black}{\textbf{0.963}} & \textcolor{black}{\textbf{0.972}} & \textcolor{red}{\textbf{1.013}} & \textcolor{red}{\textbf{1.013}} & \textcolor{black}{\textbf{0.990}} & \textcolor{black}{\textbf{0.996}} & \textcolor{black}{\textbf{0.848}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.941}} & \textcolor{black}{\textbf{0.918}} & \textcolor{black}{\textbf{0.924}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.991}} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{\textbf{0.606}} & \textcolor{black}{\textbf{0.565}} & \textcolor{black}{\textbf{0.672}}\\
\bottomrule
\end{tabular}


==> tab/geomean/geomean_groups_7.tex <==

\begin{tabular}[t]{>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|cc>{}c|ccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{2007-2010} & \multicolumn{6}{c}{2011-2014} & \multicolumn{6}{c}{2015-2019} & \multicolumn{6}{c}{2020-2022} \\
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} & \multicolumn{3}{c}{MSE} & \multicolumn{3}{c}{QLIKE} \\
 & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$ & $h=1$ & $h=5$ & $h=22$\\
\midrule
\addlinespace[0.3em]
\multicolumn{25}{c}{\textit{Panel A: DJIA index}}\\
$SV$ & \textcolor{red}{1.024} & \textcolor{red}{1.012} & \textcolor{red}{\textbf{1.002}} & \textcolor{black}{0.978} & \textcolor{black}{0.985} & \textcolor{red}{1.001} & \textcolor{black}{0.991} & \textcolor{red}{1.011} & \textcolor{black}{\textbf{0.998}} & \textcolor{black}{\textbf{0.986}} & \textcolor{black}{\textbf{0.988}} & \textcolor{black}{\textbf{0.999}} & \textcolor{red}{1.069} & \textcolor{black}{0.999} & \textcolor{red}{1.003} & \textcolor{black}{0.968} & \textcolor{black}{0.986} & \textcolor{black}{0.996} & \textcolor{red}{1.048} & \textcolor{red}{1.030} & \textcolor{red}{1.006} & \textcolor{black}{0.962} & \textcolor{black}{1.000} & \textcolor{black}{0.904}\\
$SV_{bu}$ & \textcolor{black}{0.962} & \textcolor{black}{0.991} & \textcolor{red}{1.007} & \textcolor{red}{1.024} & \textcolor{red}{1.014} & \textcolor{red}{1.011} & \textcolor{red}{1.055} & \textcolor{red}{1.016} & \textcolor{red}{1.007} & \textcolor{red}{1.069} & \textcolor{red}{1.049} & \textcolor{red}{1.014} & \textcolor{black}{0.966} & \textcolor{black}{0.985} & \textcolor{black}{0.991} & \textcolor{red}{1.021} & \textcolor{red}{1.021} & \textcolor{red}{1.004} & \textcolor{black}{0.923} & \textcolor{black}{0.921} & \textcolor{red}{\textbf{1.003}} & \textcolor{black}{0.897} & \textcolor{black}{0.051} & \textcolor{black}{0.662}\\
$SV_{shr}$ & \textcolor{black}{0.976} & \textcolor{black}{0.998} & \textcolor{red}{1.002} & \textcolor{black}{0.997} & \textcolor{black}{0.995} & \textcolor{red}{1.006} & \textcolor{red}{1.022} & \textcolor{red}{1.006} & \textcolor{red}{1.003} & \textcolor{red}{1.027} & \textcolor{red}{1.020} & \textcolor{red}{1.007} & \textcolor{black}{0.997} & \textcolor{black}{0.983} & \textcolor{black}{1.000} & \textcolor{black}{0.989} & \textcolor{black}{0.995} & \textcolor{black}{0.996} & \textcolor{black}{0.960} & \textcolor{black}{0.975} & \textcolor{red}{1.003} & \textcolor{black}{0.896} & \textcolor{black}{0.053} & \textcolor{black}{0.637}\\
$PV(3)$ & \textcolor{black}{\textbf{0.775}} & \textcolor{red}{1.047} & \textcolor{red}{1.030} & \textcolor{red}{2.691} & \textcolor{red}{1.645} & \textcolor{black}{\textbf{0.995}} & \textcolor{black}{\textbf{0.921}} & \textcolor{black}{0.973} & \textcolor{red}{1.001} & \textcolor{red}{1.073} & \textcolor{red}{1.021} & \textcolor{red}{1.011} & \textcolor{black}{0.997} & \textcolor{red}{1.013} & \textcolor{black}{0.988} & \textcolor{black}{\textbf{0.873}} & \textcolor{black}{\textbf{0.908}} & \textcolor{black}{\textbf{0.969}} & \textcolor{red}{1.059} & \textcolor{red}{1.163} & \textcolor{red}{1.012} & \textcolor{red}{6.045} & \textcolor{black}{0.942} & \textcolor{black}{0.954}\\
$PV(3)_{bu}$ & \textcolor{black}{0.922} & \textcolor{black}{\textbf{0.981}} & \textcolor{red}{1.010} & \textcolor{red}{1.023} & \textcolor{red}{1.015} & \textcolor{red}{1.011} & \textcolor{red}{1.036} & \textcolor{red}{1.013} & \textcolor{red}{1.009} & \textcolor{red}{1.076} & \textcolor{red}{1.058} & \textcolor{red}{1.021} & \textcolor{black}{0.947} & \textcolor{black}{0.979} & \textcolor{black}{0.988} & \textcolor{red}{1.004} & \textcolor{red}{1.011} & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.911}} & \textcolor{black}{\textbf{0.892}} & \textcolor{red}{1.006} & \textcolor{black}{\textbf{0.874}} & \textcolor{black}{\textbf{0.049}} & \textcolor{black}{\textbf{0.460}}\\
$PV(3)_{shr}$ & \textcolor{black}{0.812} & \textcolor{red}{1.010} & \textcolor{red}{1.018} & \textcolor{black}{\textbf{0.941}} & \textcolor{black}{\textbf{0.946}} & \textcolor{red}{1.000} & \textcolor{black}{0.944} & \textcolor{black}{\textbf{0.963}} & \textcolor{red}{1.003} & \textcolor{red}{1.047} & \textcolor{red}{1.030} & \textcolor{red}{1.015} & \textcolor{black}{\textbf{0.934}} & \textcolor{black}{\textbf{0.975}} & \textcolor{black}{\textbf{0.983}} & \textcolor{black}{0.902} & \textcolor{black}{0.938} & \textcolor{black}{0.976} & \textcolor{black}{0.947} & \textcolor{red}{1.033} & \textcolor{red}{1.005} & \textcolor{black}{0.902} & \textcolor{black}{0.051} & \textcolor{black}{0.465}\\
\addlinespace[0.3em]
\multicolumn{25}{c}{\textit{Panel B: Individual stocks}}\\
$SV$ & \textcolor{black}{0.993} & \textcolor{red}{1.014} & \textcolor{red}{1.001} & \textcolor{red}{1.124} & \textcolor{red}{1.004} & \textcolor{black}{1.000} & \textcolor{red}{1.022} & \textcolor{black}{0.985} & \textcolor{black}{0.990} & \textcolor{red}{1.076} & \textcolor{black}{0.982} & \textcolor{black}{0.988} & \textcolor{red}{1.005} & \textcolor{red}{1.001} & \textcolor{red}{1.005} & \textcolor{red}{1.080} & \textcolor{black}{0.993} & \textcolor{black}{0.997} & \textcolor{red}{1.073} & \textcolor{red}{1.005} & \textcolor{red}{1.001} & \textcolor{black}{0.963} & \textcolor{red}{1.025} & \textcolor{black}{0.994}\\
$SV_{bu}$ & \textcolor{black}{0.967} & \textcolor{black}{0.991} & \textcolor{black}{0.998} & \textcolor{red}{1.000} & \textcolor{red}{1.010} & \textcolor{red}{1.008} & \textcolor{red}{1.000} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.007} & \textcolor{red}{1.008} & \textcolor{red}{1.003} & \textcolor{black}{0.973} & \textcolor{black}{0.991} & \textcolor{black}{0.992} & \textcolor{red}{1.006} & \textcolor{black}{0.999} & \textcolor{black}{0.995} & \textcolor{black}{0.998} & \textcolor{red}{1.000} & \textcolor{red}{1.001} & \textcolor{black}{0.779} & \textcolor{black}{0.946} & \textcolor{black}{0.942}\\
$SV_{shr}$ & \textcolor{black}{0.970} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.992} & \textcolor{red}{1.001} & \textcolor{red}{1.003} & \textcolor{black}{0.985} & \textcolor{black}{0.987} & \textcolor{black}{0.993} & \textcolor{black}{0.988} & \textcolor{black}{0.991} & \textcolor{black}{0.995} & \textcolor{black}{0.979} & \textcolor{black}{0.992} & \textcolor{black}{0.995} & \textcolor{black}{0.987} & \textcolor{black}{0.990} & \textcolor{black}{0.993} & \textcolor{red}{1.029} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{black}{0.742} & \textcolor{black}{0.897} & \textcolor{black}{0.927}\\
$PV(3)$ & \textcolor{black}{0.938} & \textcolor{red}{1.035} & \textcolor{red}{1.049} & \textcolor{red}{1.421} & \textcolor{red}{1.139} & \textcolor{black}{\textbf{0.980}} & \textcolor{black}{0.973} & \textcolor{black}{0.958} & \textcolor{black}{\textbf{0.990}} & \textcolor{red}{1.046} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.976}} & \textcolor{black}{\textbf{0.836}} & \textcolor{black}{\textbf{0.943}} & \textcolor{black}{\textbf{0.941}} & \textcolor{red}{1.344} & \textcolor{red}{1.029} & \textcolor{red}{1.016} & \textcolor{red}{1.097} & \textcolor{black}{0.978} & \textcolor{black}{\textbf{0.964}} & \textcolor{red}{1.035} & \textcolor{black}{0.865} & \textcolor{red}{1.106}\\
$PV(3)_{bu}$ & \textcolor{black}{0.953} & \textcolor{black}{\textbf{0.981}} & \textcolor{black}{\textbf{0.997}} & \textcolor{red}{1.003} & \textcolor{red}{1.010} & \textcolor{red}{1.009} & \textcolor{black}{0.993} & \textcolor{black}{0.999} & \textcolor{red}{1.004} & \textcolor{red}{1.010} & \textcolor{red}{1.013} & \textcolor{red}{1.008} & \textcolor{black}{0.950} & \textcolor{black}{0.984} & \textcolor{black}{0.980} & \textcolor{black}{0.990} & \textcolor{black}{0.984} & \textcolor{black}{0.982} & \textcolor{black}{\textbf{0.994}} & \textcolor{black}{0.990} & \textcolor{black}{0.997} & \textcolor{black}{0.709} & \textcolor{black}{0.750} & \textcolor{black}{0.899}\\
$PV(3)_{shr}$ & \textcolor{black}{\textbf{0.916}} & \textcolor{black}{0.998} & \textcolor{red}{1.017} & \textcolor{black}{\textbf{0.939}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{0.983} & \textcolor{black}{\textbf{0.927}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{0.993} & \textcolor{black}{\textbf{0.970}} & \textcolor{black}{0.965} & \textcolor{black}{0.988} & \textcolor{black}{0.874} & \textcolor{black}{0.949} & \textcolor{black}{0.949} & \textcolor{black}{\textbf{0.898}} & \textcolor{black}{\textbf{0.929}} & \textcolor{black}{\textbf{0.961}} & \textcolor{red}{1.030} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{0.970} & \textcolor{black}{\textbf{0.704}} & \textcolor{black}{\textbf{0.662}} & \textcolor{black}{\textbf{0.865}}\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h22_g2.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 12.757 & 12.784 & 13.139 & 12.841 & 14.300 & 12.888 & 14.357 & 12.784 & 12.103 & 12.991 & \textbf{11.656}\\
$p$-value $dm_{RV}$ & $-$ & 0.564 & 0.828 & 0.618 & 0.932 & 0.661 & 0.940 & 0.547 & 0.102 & 0.768 & \textbf{0.026}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.831 & 0.593 & 0.934 & 0.648 & 0.943 & 0.500 & 0.069 & 0.773 & \textbf{0.013}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.230 & 0.871 & 0.272 & 0.885 & 0.176 & \textbf{0.028} & 0.260 & \textbf{0.004}\\
$p$-value MCS & \textbf{0.270} & \textbf{0.241} & \textbf{0.414} & \textbf{0.441} & \textbf{0.717} & \textbf{0.320} & \textbf{0.662} & \textbf{0.418} & 0.102 & \textbf{0.668} & \textbf{1.000}\\
\addlinespace[0.3em]
$QLIKE$ & 0.310 & 0.310 & \textbf{0.309} & 0.314 & 0.325 & 0.314 & 0.327 & 0.312 & 0.315 & 0.310 & 0.309\\
$p$-value $dm_{RV}$ & $-$ & 0.608 & 0.273 & 0.999 & 1.000 & 0.995 & 1.000 & 0.993 & 0.989 & 0.513 & 0.389\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.215 & 0.986 & 1.000 & 0.978 & 1.000 & 0.991 & 0.995 & 0.458 & 0.334\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.962 & 1.000 & 0.968 & 1.000 & 0.917 & 0.995 & 0.967 & 0.709\\
$p$-value MCS & \textbf{0.871} & \textbf{0.788} & \textbf{1.000} & \textbf{0.233} & \textbf{0.234} & \textbf{0.259} & 0.192 & \textbf{0.209} & 0.170 & \textbf{0.715} & \textbf{0.682}\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 32.313 & 32.449 & 34.051 & 32.182 & 32.879 & 32.141 & 32.731 & 32.212 & 31.604 & 32.915 & \textbf{31.458}\\
$p$-value $dm_{RV}$ & $-$ & 3 & 0 & 3 & 1 & 4 & 1 & 2 & 3 & 0 & 9\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0 & 1 & 1 & 2 & 1 & 1 & 3 & 1 & 7\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 7 & 1 & 6 & 1 & 11 & 7 & 12 & 12\\
$p$-value MCS & 26 & 25 & 26 & 25 & 23 & 26 & 25 & 26 & 24 & 25 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.250 & 0.250 & \textbf{0.244} & 0.251 & 0.259 & 0.251 & 0.260 & 0.250 & 0.251 & 0.244 & 0.245\\
$p$-value $dm_{RV}$ & $-$ & 5 & 11 & 0 & 2 & 2 & 2 & 1 & 2 & 9 & 6\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 8 & 0 & 2 & 0 & 2 & 1 & 2 & 8 & 6\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 1 & 0 & 1 & 1 & 1 & 0 & 2\\
$p$-value MCS & 20 & 20 & 26 & 20 & 10 & 17 & 11 & 18 & 11 & 22 & 22\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h22_g3.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.306 & \textbf{0.306} & 0.307 & 0.308 & 0.323 & 0.309 & 0.326 & 0.307 & 0.320 & 0.307 & 0.324\\
$p$-value $dm_{RV}$ & $-$ & 0.268 & 0.533 & 0.988 & 1.000 & 0.996 & 1.000 & 0.983 & 1.000 & 0.652 & 0.996\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.576 & 0.944 & 1.000 & 0.972 & 1.000 & 0.902 & 1.000 & 0.730 & 0.997\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.627 & 0.998 & 0.681 & 0.999 & 0.539 & 0.992 & 0.550 & 0.997\\
$p$-value MCS & \textbf{0.463} & \textbf{1.000} & \textbf{0.940} & \textbf{0.347} & 0.081 & \textbf{0.213} & 0.176 & \textbf{0.845} & 0.189 & \textbf{0.779} & \textbf{0.295}\\
\addlinespace[0.3em]
$QLIKE$ & 0.201 & \textbf{0.201} & 0.203 & 0.204 & 0.220 & 0.205 & 0.222 & 0.203 & 0.212 & 0.204 & 0.207\\
$p$-value $dm_{RV}$ & $-$ & 0.217 & 0.995 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.998 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.760 & 1.000 & 0.990 & 1.000 & 0.176 & 1.000 & 0.959 & 1.000\\
$p$-value MCS & \textbf{0.404} & \textbf{1.000} & 0.126 & 0.008 & 0.000 & 0.001 & 0.000 & 0.133 & 0.001 & 0.002 & 0.001\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 0.983 & 0.972 & \textbf{0.971} & 0.985 & 1.029 & 0.986 & 1.041 & 0.976 & 0.997 & 0.975 & 0.991\\
$p$-value $dm_{RV}$ & $-$ & 8 & 8 & 2 & 1 & 2 & 1 & 6 & 1 & 9 & 4\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 7 & 0 & 1 & 0 & 1 & 2 & 1 & 8 & 2\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 3 & 1 & 3 & 1 & 4 & 1 & 4 & 1\\
$p$-value MCS & 18 & 25 & 22 & 15 & 7 & 13 & 11 & 16 & 10 & 15 & 14\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.118 & 0.116 & \textbf{0.114} & 0.118 & 0.122 & 0.118 & 0.123 & 0.117 & 0.119 & 0.115 & 0.116\\
$p$-value $dm_{RV}$ & $-$ & 12 & 17 & 1 & 1 & 1 & 1 & 8 & 1 & 14 & 7\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 16 & 0 & 1 & 0 & 1 & 0 & 1 & 10 & 5\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 0 & 1 & 2 & 1 & 1 & 1\\
$p$-value MCS & 13 & 16 & 23 & 8 & 2 & 5 & 2 & 9 & 2 & 9 & 9\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h22_g4.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.249 & 0.250 & 0.246 & 0.247 & 0.247 & 0.246 & 0.247 & 0.249 & 0.251 & \textbf{0.245} & 0.247\\
$p$-value $dm_{RV}$ & $-$ & 0.707 & 0.210 & 0.090 & 0.133 & \textbf{0.041} & 0.152 & 0.468 & 0.842 & \textbf{0.022} & 0.126\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.181 & 0.163 & 0.176 & 0.110 & 0.188 & \textbf{0.027} & 0.681 & \textbf{0.040} & 0.130\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.587 & 0.574 & 0.496 & 0.589 & 0.765 & 0.873 & 0.227 & 0.578\\
$p$-value MCS & \textbf{0.668} & \textbf{0.666} & \textbf{0.939} & \textbf{0.961} & \textbf{0.911} & \textbf{0.575} & \textbf{0.955} & \textbf{0.686} & \textbf{0.503} & \textbf{1.000} & \textbf{0.945}\\
\addlinespace[0.3em]
$QLIKE$ & 0.335 & 0.334 & \textbf{0.325} & 0.336 & 0.337 & 0.335 & 0.337 & 0.334 & 0.334 & 0.327 & 0.327\\
$p$-value $dm_{RV}$ & $-$ & 0.143 & \textbf{0.000} & 0.918 & 0.908 & 0.494 & 0.934 & 0.159 & 0.201 & \textbf{0.000} & \textbf{0.000}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & \textbf{0.000} & 0.914 & 0.929 & 0.750 & 0.945 & 0.674 & 0.630 & \textbf{0.000} & \textbf{0.000}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.998 & 0.996\\
$p$-value MCS & 0.101 & 0.048 & \textbf{1.000} & 0.104 & 0.139 & 0.090 & 0.135 & 0.036 & 0.069 & \textbf{0.251} & 0.089\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 1.495 & 1.490 & \textbf{1.229} & 1.454 & 1.280 & 1.409 & 1.263 & 1.464 & 1.357 & 1.294 & 1.261\\
$p$-value $dm_{RV}$ & $-$ & 1 & 12 & 2 & 5 & 13 & 5 & 4 & 10 & 12 & 11\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 11 & 1 & 3 & 4 & 3 & 1 & 5 & 11 & 11\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 2\\
$p$-value MCS & 20 & 23 & 25 & 18 & 20 & 19 & 24 & 22 & 21 & 23 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.160 & 0.159 & 0.163 & 0.158 & 0.152 & 0.154 & 0.152 & 0.158 & 0.153 & 0.151 & \textbf{0.149}\\
$p$-value $dm_{RV}$ & $-$ & 5 & 8 & 6 & 10 & 13 & 10 & 6 & 11 & 16 & 17\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 9 & 2 & 9 & 8 & 9 & 2 & 9 & 14 & 17\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 2 & 2 & 2 & 1 & 2 & 2 & 2\\
$p$-value MCS & 13 & 13 & 26 & 15 & 16 & 14 & 15 & 14 & 13 & 20 & 24\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h22_g5.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & \textbf{6.057} & 6.091 & 6.130 & 6.074 & 6.268 & 6.092 & 6.283 & 6.076 & 6.119 & 6.088 & 6.132\\
$p$-value $dm_{RV}$ & $-$ & 0.805 & 0.831 & 0.822 & 0.965 & 0.845 & 0.965 & 0.798 & 0.855 & 0.749 & 0.824\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.805 & 0.300 & 0.944 & 0.505 & 0.948 & 0.242 & 0.708 & 0.448 & 0.741\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.204 & 0.879 & 0.266 & 0.895 & 0.180 & 0.438 & 0.133 & 0.514\\
$p$-value MCS & \textbf{1.000} & \textbf{0.894} & \textbf{0.897} & \textbf{0.595} & \textbf{0.717} & \textbf{0.834} & \textbf{0.726} & \textbf{0.697} & \textbf{0.914} & \textbf{0.720} & \textbf{0.879}\\
\addlinespace[0.3em]
$QLIKE$ & 4.668 & 4.221 & 4.455 & 3.089 & 0.793 & 2.146 & 0.788 & 2.975 & \textbf{0.787} & 2.172 & 0.787\\
$p$-value $dm_{RV}$ & $-$ & 0.161 & 0.173 & \textbf{0.026} & \textbf{0.000} & \textbf{0.002} & \textbf{0.000} & \textbf{0.016} & \textbf{0.000} & \textbf{0.002} & \textbf{0.000}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.849 & \textbf{0.047} & \textbf{0.000} & \textbf{0.003} & \textbf{0.000} & \textbf{0.028} & \textbf{0.000} & \textbf{0.003} & \textbf{0.000}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & \textbf{0.028} & \textbf{0.000} & \textbf{0.002} & \textbf{0.000} & \textbf{0.016} & \textbf{0.000} & \textbf{0.002} & \textbf{0.000}\\
$p$-value MCS & \textbf{0.280} & \textbf{0.393} & \textbf{0.374} & \textbf{0.340} & \textbf{0.803} & \textbf{0.335} & \textbf{0.991} & \textbf{0.339} & \textbf{1.000} & \textbf{0.345} & \textbf{0.837}\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 32.599 & 32.625 & 30.757 & 32.658 & 30.553 & 32.979 & 30.132 & 32.614 & 29.727 & 31.259 & \textbf{28.197}\\
$p$-value $dm_{RV}$ & $-$ & 2 & 10 & 1 & 3 & 7 & 4 & 2 & 4 & 12 & 10\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 11 & 4 & 4 & 5 & 4 & 3 & 5 & 11 & 11\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 0 & 1 & 0 & 1 & 1 & 2 & 2\\
$p$-value MCS & 22 & 23 & 25 & 22 & 26 & 23 & 24 & 21 & 25 & 23 & 25\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.778 & 0.773 & 0.932 & 0.734 & 0.505 & 0.700 & 0.489 & 0.717 & 0.487 & 0.669 & \textbf{0.463}\\
$p$-value $dm_{RV}$ & $-$ & 1 & 6 & 5 & 14 & 10 & 15 & 6 & 14 & 17 & 21\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 6 & 5 & 13 & 10 & 15 & 6 & 16 & 14 & 21\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 10 & 15 & 10 & 15 & 13 & 17 & 14 & 17\\
$p$-value MCS & 24 & 23 & 25 & 24 & 25 & 25 & 25 & 24 & 23 & 25 & 25\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h5_g2.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 13.355 & 13.519 & 13.983 & 13.236 & 10.335 & 13.107 & \textbf{10.227} & 13.325 & 11.397 & 13.493 & 12.135\\
$p$-value $dm_{RV}$ & $-$ & 0.663 & 0.663 & 0.254 & \textbf{0.005} & 0.121 & \textbf{0.005} & 0.439 & \textbf{0.002} & 0.556 & 0.069\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.623 & 0.263 & \textbf{0.007} & 0.178 & \textbf{0.006} & 0.234 & \textbf{0.003} & 0.490 & 0.061\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.313 & \textbf{0.044} & 0.281 & \textbf{0.041} & 0.329 & 0.072 & 0.190 & \textbf{0.032}\\
$p$-value MCS & \textbf{0.347} & \textbf{0.385} & \textbf{0.410} & \textbf{0.261} & \textbf{0.314} & \textbf{0.267} & \textbf{1.000} & \textbf{0.338} & \textbf{0.488} & \textbf{0.452} & \textbf{0.445}\\
\addlinespace[0.3em]
$QLIKE$ & 0.176 & 0.173 & 0.290 & 0.179 & 0.187 & 0.179 & 0.188 & 0.175 & 0.178 & \textbf{0.167} & 0.168\\
$p$-value $dm_{RV}$ & $-$ & 0.058 & 0.817 & 0.993 & 1.000 & 0.990 & 1.000 & 0.178 & 0.855 & \textbf{0.000} & \textbf{0.000}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.822 & 0.989 & 1.000 & 0.989 & 1.000 & 0.945 & 0.989 & \textbf{0.000} & \textbf{0.009}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.188 & 0.208 & 0.189 & 0.209 & 0.181 & 0.186 & 0.164 & 0.167\\
$p$-value MCS & 0.005 & 0.023 & \textbf{0.634} & 0.005 & 0.024 & 0.003 & 0.020 & 0.007 & 0.001 & \textbf{1.000} & 0.042\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 47.181 & 50.701 & 49.773 & 46.686 & 59.282 & \textbf{46.091} & 57.108 & 48.366 & 50.043 & 47.826 & 47.637\\
$p$-value $dm_{RV}$ & $-$ & 1 & 0 & 2 & 7 & 5 & 8 & 2 & 9 & 2 & 6\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0 & 1 & 6 & 5 & 7 & 1 & 8 & 1 & 5\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 2 & 0 & 2 & 0 & 2 & 2 & 5\\
$p$-value MCS & 26 & 25 & 26 & 26 & 23 & 26 & 26 & 26 & 26 & 26 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.161 & 0.161 & 0.264 & 0.162 & 0.170 & 0.162 & 0.170 & 0.161 & 0.162 & \textbf{0.152} & 0.153\\
$p$-value $dm_{RV}$ & $-$ & 3 & 7 & 0 & 1 & 1 & 1 & 1 & 1 & 16 & 14\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 5 & 0 & 1 & 0 & 1 & 0 & 0 & 12 & 11\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 1 & 1 & 1 & 1 & 3 & 3\\
$p$-value MCS & 17 & 23 & 26 & 13 & 2 & 13 & 4 & 20 & 8 & 23 & 18\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h5_g3.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.344 & 0.348 & 0.335 & 0.350 & 0.369 & 0.349 & 0.371 & 0.346 & 0.355 & \textbf{0.331} & 0.339\\
$p$-value $dm_{RV}$ & $-$ & 0.660 & 0.381 & 0.960 & 0.999 & 0.908 & 0.999 & 0.777 & 0.994 & 0.235 & 0.370\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.323 & 0.557 & 0.928 & 0.520 & 0.942 & 0.395 & 0.740 & 0.169 & 0.279\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.675 & 0.824 & 0.664 & 0.834 & 0.642 & 0.724 & 0.404 & 0.604\\
$p$-value MCS & \textbf{0.689} & \textbf{0.624} & \textbf{0.622} & \textbf{0.564} & 0.087 & \textbf{0.588} & 0.064 & \textbf{0.733} & \textbf{0.318} & \textbf{1.000} & \textbf{0.792}\\
\addlinespace[0.3em]
$QLIKE$ & 0.164 & \textbf{0.162} & 0.167 & 0.172 & 0.198 & 0.173 & 0.202 & 0.167 & 0.179 & 0.169 & 0.174\\
$p$-value $dm_{RV}$ & $-$ & \textbf{0.034} & 0.888 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.995 & 1.000\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.984 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.926 & 1.000 & 0.974 & 1.000 & 0.473 & 1.000 & 0.905 & 1.000\\
$p$-value MCS & 0.028 & \textbf{1.000} & \textbf{0.407} & 0.016 & 0.000 & 0.011 & 0.000 & 0.176 & 0.000 & 0.118 & 0.004\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 1.024 & 1.011 & \textbf{0.961} & 1.024 & 1.068 & 1.020 & 1.076 & 1.013 & 1.032 & 0.970 & 0.993\\
$p$-value $dm_{RV}$ & $-$ & 3 & 3 & 2 & 1 & 3 & 1 & 5 & 2 & 8 & 5\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 5 & 0 & 1 & 0 & 1 & 0 & 1 & 6 & 3\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 0 & 1 & 0 & 2 & 0 & 3 & 1\\
$p$-value MCS & 19 & 21 & 24 & 18 & 5 & 18 & 6 & 17 & 8 & 22 & 19\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.105 & 0.102 & \textbf{0.097} & 0.105 & 0.113 & 0.106 & 0.114 & 0.103 & 0.107 & 0.100 & 0.102\\
$p$-value $dm_{RV}$ & $-$ & 12 & 12 & 1 & 1 & 1 & 1 & 9 & 3 & 15 & 7\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 10 & 0 & 1 & 0 & 1 & 1 & 1 & 9 & 4\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 0 & 1 & 0 & 3 & 0 & 4 & 2\\
$p$-value MCS & 13 & 16 & 25 & 10 & 0 & 6 & 1 & 10 & 0 & 17 & 6\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h5_g4.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.432 & 0.432 & 0.438 & 0.425 & 0.422 & 0.423 & 0.422 & 0.425 & 0.418 & 0.421 & \textbf{0.415}\\
$p$-value $dm_{RV}$ & $-$ & 0.468 & 0.596 & 0.133 & 0.106 & 0.073 & 0.113 & \textbf{0.014} & \textbf{0.013} & 0.174 & 0.060\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.598 & 0.244 & 0.176 & 0.172 & 0.185 & 0.131 & 0.055 & 0.211 & 0.093\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.301 & 0.259 & 0.259 & 0.264 & 0.287 & 0.198 & 0.102 & 0.077\\
$p$-value MCS & \textbf{0.639} & \textbf{0.761} & \textbf{0.809} & \textbf{0.499} & \textbf{0.745} & \textbf{0.770} & \textbf{0.704} & \textbf{0.579} & \textbf{0.748} & \textbf{0.731} & \textbf{1.000}\\
\addlinespace[0.3em]
$QLIKE$ & 0.277 & 0.273 & \textbf{0.251} & 0.283 & 0.289 & 0.280 & 0.290 & 0.275 & 0.276 & 0.260 & 0.262\\
$p$-value $dm_{RV}$ & $-$ & \textbf{0.007} & \textbf{0.000} & 0.979 & 0.999 & 0.861 & 1.000 & \textbf{0.035} & 0.370 & \textbf{0.000} & \textbf{0.001}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & \textbf{0.002} & 0.988 & 0.999 & 0.946 & 0.999 & 0.986 & 0.975 & \textbf{0.004} & \textbf{0.013}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1.000 & 1.000 & 1.000 & 1.000 & 0.999 & 1.000 & 0.998 & 0.999\\
$p$-value MCS & 0.088 & 0.153 & \textbf{1.000} & 0.069 & 0.026 & 0.079 & 0.017 & 0.059 & 0.032 & 0.045 & 0.010\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 4.503 & 4.424 & \textbf{3.793} & 4.380 & 5.215 & 4.431 & 5.319 & 4.384 & 4.770 & 4.099 & 4.672\\
$p$-value $dm_{RV}$ & $-$ & 4 & 8 & 2 & 4 & 6 & 3 & 7 & 9 & 13 & 17\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 9 & 0 & 3 & 4 & 3 & 1 & 2 & 12 & 14\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2\\
$p$-value MCS & 13 & 19 & 25 & 14 & 17 & 14 & 18 & 17 & 18 & 24 & 25\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.176 & 0.174 & 0.182 & 0.175 & 0.170 & 0.171 & 0.170 & 0.173 & 0.169 & 0.160 & \textbf{0.159}\\
$p$-value $dm_{RV}$ & $-$ & 7 & 9 & 4 & 7 & 12 & 7 & 9 & 11 & 25 & 25\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 8 & 0 & 4 & 3 & 4 & 0 & 6 & 23 & 24\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 1 & 1 & 2 & 0 & 1 & 3 & 3\\
$p$-value MCS & 3 & 11 & 25 & 3 & 3 & 5 & 4 & 6 & 3 & 20 & 20\\
\bottomrule
\end{tabular}


==> tab_com/tab_com_h5_g5.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|ccc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $TSV_{bu}$ & $PV(3)_{bu}$ & $TPV(3)_{bu}$ & $SV_{shr}$ & $TSV_{shr}$ & $PV(3)_{shr}$ & $TPV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 8.894 & 9.159 & 10.340 & 8.196 & 7.407 & 7.929 & \textbf{7.398} & 8.673 & 8.184 & 9.186 & 8.500\\
$p$-value $dm_{RV}$ & $-$ & 0.786 & 0.964 & \textbf{0.017} & 0.073 & \textbf{0.015} & 0.084 & 0.170 & \textbf{0.029} & 0.766 & 0.158\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.985 & \textbf{0.031} & 0.053 & \textbf{0.025} & 0.062 & \textbf{0.020} & \textbf{0.010} & 0.563 & \textbf{0.016}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & \textbf{0.019} & \textbf{0.028} & \textbf{0.017} & \textbf{0.032} & \textbf{0.014} & \textbf{0.009} & \textbf{0.010} & \textbf{0.007}\\
$p$-value MCS & \textbf{0.568} & \textbf{0.426} & \textbf{0.531} & \textbf{0.403} & \textbf{0.738} & \textbf{0.561} & \textbf{1.000} & \textbf{0.411} & \textbf{0.433} & \textbf{0.480} & \textbf{0.424}\\
\addlinespace[0.3em]
$QLIKE$ & 4.692 & 4.691 & 4.419 & 0.241 & 0.240 & \textbf{0.232} & 0.238 & 0.247 & 0.235 & 0.241 & 0.234\\
$p$-value $dm_{RV}$ & $-$ & 0.121 & 0.381 & \textbf{0.007} & \textbf{0.008} & \textbf{0.007} & \textbf{0.008} & \textbf{0.007} & \textbf{0.007} & \textbf{0.007} & \textbf{0.007}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.381 & \textbf{0.007} & \textbf{0.008} & \textbf{0.007} & \textbf{0.008} & \textbf{0.007} & \textbf{0.007} & \textbf{0.007} & \textbf{0.007}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & \textbf{0.008} & \textbf{0.008} & \textbf{0.008} & \textbf{0.008} & \textbf{0.008} & \textbf{0.008} & \textbf{0.008} & \textbf{0.008}\\
$p$-value MCS & \textbf{0.475} & \textbf{0.472} & \textbf{0.477} & \textbf{0.871} & \textbf{0.687} & \textbf{1.000} & \textbf{0.926} & \textbf{0.834} & \textbf{0.585} & \textbf{0.861} & \textbf{0.789}\\
\midrule
\addlinespace[0.3em]
\multicolumn{12}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 69.753 & 65.892 & \textbf{53.554} & 68.896 & 72.606 & 67.445 & 70.494 & 66.938 & 68.458 & 54.923 & 56.730\\
$p$-value $dm_{RV}$ & $-$ & 0 & 4 & 1 & 0 & 4 & 0 & 2 & 0 & 5 & 7\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 3 & 3 & 0 & 2 & 3 & 3 & 2 & 6 & 6\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 0 & 1 & 1 & 2 & 1 & 1 & 2\\
$p$-value MCS & 26 & 26 & 26 & 26 & 25 & 26 & 26 & 26 & 26 & 26 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.379 & 0.389 & 0.307 & 0.345 & 0.209 & 0.227 & 0.205 & 0.309 & 0.181 & 0.189 & \textbf{0.148}\\
$p$-value $dm_{RV}$ & $-$ & 2 & 9 & 5 & 5 & 10 & 5 & 6 & 9 & 15 & 16\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 8 & 7 & 5 & 9 & 5 & 10 & 11 & 18 & 21\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 4 & 6 & 7 & 6 & 2 & 9 & 13 & 14\\
$p$-value MCS & 21 & 18 & 22 & 22 & 24 & 23 & 26 & 21 & 20 & 21 & 25\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h1_g2.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 20.587 & 21.074 & \textbf{15.957} & 19.808 & 18.972 & 20.097 & 16.718\\
$p$-value $dm_{RV}$ & $-$ & 0.718 & 0.162 & 0.197 & 0.107 & 0.159 & 0.077\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.135 & 0.211 & 0.121 & 0.174 & 0.060\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.820 & 0.789 & 0.833 & 0.639\\
$p$-value MCS & \textbf{0.332} & \textbf{0.332} & \textbf{1.000} & \textbf{0.299} & \textbf{0.337} & \textbf{0.327} & \textbf{0.491}\\
\addlinespace[0.3em]
$QLIKE$ & 0.187 & 0.183 & 0.505 & 0.192 & 0.192 & 0.187 & \textbf{0.176}\\
$p$-value $dm_{RV}$ & $-$ & \textbf{0.002} & 0.873 & 0.999 & 0.996 & 0.267 & \textbf{0.001}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.876 & 1.000 & 1.000 & 0.999 & \textbf{0.024}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.131 & 0.131 & 0.127 & 0.119\\
$p$-value MCS & 0.004 & 0.057 & 0.125 & 0.000 & 0.000 & 0.007 & \textbf{1.000}\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 96.815 & 97.020 & 95.505 & 93.645 & 92.522 & 94.130 & \textbf{91.192}\\
$p$-value $dm_{RV}$ & $-$ & 0 & 0 & 0 & 2 & 0 & 3\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0 & 1 & 1 & 2 & 3\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 1 & 1\\
$p$-value MCS & 25 & 24 & 26 & 19 & 26 & 24 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.196 & 0.224 & 0.287 & 0.188 & 0.191 & 0.187 & \textbf{0.166}\\
$p$-value $dm_{RV}$ & $-$ & 4 & 0 & 0 & 1 & 3 & 13\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 1 & 1 & 0 & 3 & 9\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 4 & 3 & 5 & 6\\
$p$-value MCS & 12 & 15 & 18 & 7 & 8 & 14 & 26\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h1_g3.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.433 & 0.429 & \textbf{0.399} & 0.457 & 0.449 & 0.442 & 0.409\\
$p$-value $dm_{RV}$ & $-$ & 0.339 & 0.242 & 0.991 & 0.942 & 0.995 & 0.100\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.266 & 0.929 & 0.849 & 0.866 & 0.184\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.860 & 0.834 & 0.803 & 0.621\\
$p$-value MCS & \textbf{0.462} & \textbf{0.637} & \textbf{1.000} & 0.099 & 0.089 & \textbf{0.272} & \textbf{0.672}\\
\addlinespace[0.3em]
$QLIKE$ & 0.195 & \textbf{0.192} & 0.209 & 0.209 & 0.210 & 0.200 & 0.204\\
$p$-value $dm_{RV}$ & $-$ & \textbf{0.003} & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.423 & 0.555 & \textbf{0.014} & \textbf{0.025}\\
$p$-value MCS & 0.006 & \textbf{1.000} & 0.038 & 0.006 & 0.001 & 0.000 & 0.025\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 1.508 & 1.568 & 1.464 & 1.504 & 1.492 & 1.494 & \textbf{1.404}\\
$p$-value $dm_{RV}$ & $-$ & 1 & 4 & 3 & 5 & 7 & 9\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 3 & 1 & 1 & 4 & 10\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 0 & 2\\
$p$-value MCS & 21 & 19 & 24 & 21 & 20 & 19 & 25\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.123 & 0.148 & 0.133 & 0.124 & 0.124 & 0.121 & \textbf{0.118}\\
$p$-value $dm_{RV}$ & $-$ & 8 & 4 & 1 & 1 & 10 & 14\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 5 & 3 & 3 & 5 & 9\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 6 & 6 & 9 & 14\\
$p$-value MCS & 14 & 16 & 16 & 8 & 6 & 14 & 22\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h1_g4.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.901 & 0.963 & 0.899 & 0.871 & 0.854 & 0.898 & \textbf{0.841}\\
$p$-value $dm_{RV}$ & $-$ & 0.830 & 0.485 & 0.145 & 0.113 & 0.384 & 0.103\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.294 & 0.155 & 0.141 & 0.139 & 0.124\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.324 & 0.216 & 0.498 & 0.056\\
$p$-value MCS & \textbf{0.804} & \textbf{0.651} & \textbf{0.701} & \textbf{0.382} & \textbf{0.577} & \textbf{0.823} & \textbf{1.000}\\
\addlinespace[0.3em]
$QLIKE$ & 0.242 & 0.234 & \textbf{0.211} & 0.247 & 0.243 & 0.239 & 0.218\\
$p$-value $dm_{RV}$ & $-$ & \textbf{0.012} & \textbf{0.008} & 0.866 & 0.597 & \textbf{0.023} & \textbf{0.001}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & \textbf{0.024} & 0.951 & 0.893 & 0.977 & \textbf{0.006}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.987 & 0.984 & 0.986 & 0.875\\
$p$-value MCS & 0.013 & 0.031 & \textbf{1.000} & 0.034 & 0.050 & 0.046 & \textbf{0.228}\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 28.790 & 28.277 & \textbf{13.400} & 25.753 & 24.144 & 26.345 & 17.863\\
$p$-value $dm_{RV}$ & $-$ & 2 & 1 & 0 & 3 & 4 & 9\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 3 & 1 & 1 & 2 & 7\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 0 & 0\\
$p$-value MCS & 16 & 18 & 25 & 15 & 17 & 20 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.183 & 0.239 & 0.345 & 0.184 & 0.179 & 0.179 & \textbf{0.159}\\
$p$-value $dm_{RV}$ & $-$ & 2 & 5 & 1 & 7 & 5 & 25\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 7 & 2 & 4 & 5 & 24\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 3 & 3 & 4 & 7\\
$p$-value MCS & 1 & 3 & 20 & 3 & 1 & 2 & 24\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h1_g5.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 3.910 & 4.096 & 4.141 & 3.610 & \textbf{3.561} & 3.752 & 3.702\\
$p$-value $dm_{RV}$ & $-$ & 0.838 & 0.854 & \textbf{0.012} & \textbf{0.011} & 0.076 & 0.057\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.605 & \textbf{0.016} & \textbf{0.013} & \textbf{0.015} & \textbf{0.019}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & \textbf{0.017} & \textbf{0.012} & \textbf{0.028} & \textbf{0.009}\\
$p$-value MCS & \textbf{0.475} & \textbf{0.406} & 0.153 & 0.075 & \textbf{1.000} & \textbf{0.287} & \textbf{0.252}\\
\addlinespace[0.3em]
$QLIKE$ & 0.245 & 0.236 & 1.482 & 0.220 & \textbf{0.214} & 0.220 & 0.221\\
$p$-value $dm_{RV}$ & $-$ & 0.206 & 0.847 & 0.160 & 0.128 & 0.153 & 0.176\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.847 & 0.133 & 0.090 & 0.120 & 0.158\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.153 & 0.152 & 0.153 & 0.153\\
$p$-value MCS & \textbf{0.622} & \textbf{0.573} & 0.125 & 0.030 & \textbf{1.000} & 0.155 & 0.007\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 30.422 & 39.697 & 43.397 & 30.482 & \textbf{30.197} & 35.764 & 36.386\\
$p$-value $dm_{RV}$ & $-$ & 0 & 0 & 1 & 3 & 0 & 0\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 1 & 3 & 4 & 3 & 2\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 2 & 2\\
$p$-value MCS & 24 & 25 & 25 & 24 & 25 & 24 & 25\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.269 & 0.256 & 0.305 & 0.186 & 0.163 & 0.172 & \textbf{0.162}\\
$p$-value $dm_{RV}$ & $-$ & 0 & 4 & 2 & 3 & 1 & 10\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 9 & 6 & 7 & 6 & 13\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 3 & 5 & 5 & 9\\
$p$-value MCS & 19 & 16 & 22 & 15 & 19 & 13 & 21\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h22_g2.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & \textbf{12.757} & 12.784 & 13.139 & 12.841 & 12.888 & 12.784 & 12.991\\
$p$-value $dm_{RV}$ & $-$ & 0.564 & 0.828 & 0.618 & 0.661 & 0.547 & 0.768\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.831 & 0.593 & 0.648 & 0.500 & 0.773\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.230 & 0.272 & 0.176 & 0.260\\
$p$-value MCS & \textbf{1.000} & \textbf{0.960} & \textbf{0.763} & \textbf{0.799} & \textbf{0.860} & \textbf{0.804} & \textbf{0.816}\\
\addlinespace[0.3em]
$QLIKE$ & 0.310 & 0.310 & \textbf{0.309} & 0.314 & 0.314 & 0.312 & 0.310\\
$p$-value $dm_{RV}$ & $-$ & 0.608 & 0.273 & 0.999 & 0.995 & 0.993 & 0.513\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.215 & 0.986 & 0.978 & 0.991 & 0.458\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.962 & 0.968 & 0.917 & 0.967\\
$p$-value MCS & \textbf{0.589} & \textbf{0.798} & \textbf{1.000} & 0.076 & 0.146 & 0.108 & \textbf{0.491}\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 32.313 & 32.449 & 34.051 & 32.182 & \textbf{32.141} & 32.212 & 32.915\\
$p$-value $dm_{RV}$ & $-$ & 3 & 0 & 3 & 4 & 2 & 0\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0 & 1 & 2 & 1 & 1\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 7 & 6 & 11 & 12\\
$p$-value MCS & 25 & 26 & 25 & 24 & 26 & 24 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.250 & 0.250 & \textbf{0.244} & 0.251 & 0.251 & 0.250 & 0.244\\
$p$-value $dm_{RV}$ & $-$ & 5 & 11 & 0 & 2 & 1 & 9\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 8 & 0 & 0 & 1 & 8\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 1 & 0\\
$p$-value MCS & 20 & 20 & 26 & 12 & 15 & 16 & 21\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h22_g3.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.306 & \textbf{0.306} & 0.307 & 0.308 & 0.309 & 0.307 & 0.307\\
$p$-value $dm_{RV}$ & $-$ & 0.268 & 0.533 & 0.988 & 0.996 & 0.983 & 0.652\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.576 & 0.944 & 0.972 & 0.902 & 0.730\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.627 & 0.681 & 0.539 & 0.550\\
$p$-value MCS & \textbf{0.459} & \textbf{1.000} & \textbf{0.939} & \textbf{0.337} & \textbf{0.214} & \textbf{0.839} & \textbf{0.778}\\
\addlinespace[0.3em]
$QLIKE$ & 0.201 & \textbf{0.201} & 0.203 & 0.204 & 0.205 & 0.203 & 0.204\\
$p$-value $dm_{RV}$ & $-$ & 0.217 & 0.995 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.998 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.760 & 0.990 & 0.176 & 0.959\\
$p$-value MCS & \textbf{0.415} & \textbf{1.000} & 0.127 & 0.008 & 0.000 & 0.144 & 0.002\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 0.983 & 0.972 & \textbf{0.971} & 0.985 & 0.986 & 0.976 & 0.975\\
$p$-value $dm_{RV}$ & $-$ & 8 & 8 & 2 & 2 & 6 & 9\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 7 & 0 & 0 & 2 & 8\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 3 & 3 & 4 & 4\\
$p$-value MCS & 16 & 20 & 23 & 13 & 13 & 12 & 15\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.118 & 0.116 & \textbf{0.114} & 0.118 & 0.118 & 0.117 & 0.115\\
$p$-value $dm_{RV}$ & $-$ & 12 & 17 & 1 & 1 & 8 & 14\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 16 & 0 & 0 & 0 & 10\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 0 & 2 & 1\\
$p$-value MCS & 12 & 14 & 24 & 6 & 5 & 8 & 7\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h22_g4.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.249 & 0.250 & 0.246 & 0.247 & 0.246 & 0.249 & \textbf{0.245}\\
$p$-value $dm_{RV}$ & $-$ & 0.707 & 0.210 & 0.090 & \textbf{0.041} & 0.468 & \textbf{0.022}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.181 & 0.163 & 0.110 & \textbf{0.027} & \textbf{0.040}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.587 & 0.496 & 0.765 & 0.227\\
$p$-value MCS & \textbf{0.437} & \textbf{0.419} & \textbf{0.946} & \textbf{0.760} & \textbf{0.572} & \textbf{0.434} & \textbf{1.000}\\
\addlinespace[0.3em]
$QLIKE$ & 0.335 & 0.334 & \textbf{0.325} & 0.336 & 0.335 & 0.334 & 0.327\\
$p$-value $dm_{RV}$ & $-$ & 0.143 & \textbf{0.000} & 0.918 & 0.494 & 0.159 & \textbf{0.000}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & \textbf{0.000} & 0.914 & 0.750 & 0.674 & \textbf{0.000}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1.000 & 1.000 & 1.000 & 0.998\\
$p$-value MCS & 0.064 & 0.028 & \textbf{1.000} & 0.051 & 0.102 & 0.024 & 0.044\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 1.495 & 1.490 & \textbf{1.229} & 1.454 & 1.409 & 1.464 & 1.294\\
$p$-value $dm_{RV}$ & $-$ & 1 & 12 & 2 & 13 & 4 & 12\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 11 & 1 & 4 & 1 & 11\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 0 & 1\\
$p$-value MCS & 13 & 16 & 26 & 13 & 15 & 14 & 23\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.160 & 0.159 & 0.163 & 0.158 & 0.154 & 0.158 & \textbf{0.151}\\
$p$-value $dm_{RV}$ & $-$ & 5 & 8 & 6 & 13 & 6 & 16\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 9 & 2 & 8 & 2 & 14\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 2 & 1 & 2\\
$p$-value MCS & 11 & 15 & 26 & 11 & 13 & 11 & 22\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h22_g5.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & \textbf{6.057} & 6.091 & 6.130 & 6.074 & 6.092 & 6.076 & 6.088\\
$p$-value $dm_{RV}$ & $-$ & 0.805 & 0.831 & 0.822 & 0.845 & 0.798 & 0.749\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.805 & 0.300 & 0.505 & 0.242 & 0.448\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.204 & 0.266 & 0.180 & 0.133\\
$p$-value MCS & \textbf{1.000} & \textbf{0.896} & \textbf{0.794} & \textbf{0.608} & \textbf{0.848} & \textbf{0.699} & \textbf{0.734}\\
\addlinespace[0.3em]
$QLIKE$ & 4.668 & 4.221 & 4.455 & 3.089 & \textbf{2.146} & 2.975 & 2.172\\
$p$-value $dm_{RV}$ & $-$ & 0.161 & 0.173 & \textbf{0.026} & \textbf{0.002} & \textbf{0.016} & \textbf{0.002}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.849 & \textbf{0.047} & \textbf{0.003} & \textbf{0.028} & \textbf{0.003}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & \textbf{0.028} & \textbf{0.002} & \textbf{0.016} & \textbf{0.002}\\
$p$-value MCS & \textbf{0.250} & \textbf{0.263} & \textbf{0.260} & \textbf{0.232} & \textbf{1.000} & \textbf{0.358} & \textbf{0.401}\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 32.599 & 32.625 & \textbf{30.757} & 32.658 & 32.979 & 32.614 & 31.259\\
$p$-value $dm_{RV}$ & $-$ & 2 & 10 & 1 & 7 & 2 & 12\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 11 & 4 & 5 & 3 & 11\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 1 & 2\\
$p$-value MCS & 18 & 18 & 24 & 21 & 20 & 21 & 22\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.778 & 0.773 & 0.932 & 0.734 & 0.700 & 0.717 & \textbf{0.669}\\
$p$-value $dm_{RV}$ & $-$ & 1 & 6 & 5 & 10 & 6 & 17\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 6 & 5 & 10 & 6 & 14\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 10 & 10 & 13 & 14\\
$p$-value MCS & 26 & 20 & 22 & 24 & 25 & 23 & 23\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h5_g2.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 13.355 & 13.519 & 13.983 & 13.236 & \textbf{13.107} & 13.325 & 13.493\\
$p$-value $dm_{RV}$ & $-$ & 0.663 & 0.663 & 0.254 & 0.121 & 0.439 & 0.556\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.623 & 0.263 & 0.178 & 0.234 & 0.490\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.313 & 0.281 & 0.329 & 0.190\\
$p$-value MCS & \textbf{0.876} & \textbf{0.732} & \textbf{0.739} & 0.126 & \textbf{1.000} & \textbf{0.644} & \textbf{0.816}\\
\addlinespace[0.3em]
$QLIKE$ & 0.176 & 0.173 & 0.290 & 0.179 & 0.179 & 0.175 & \textbf{0.167}\\
$p$-value $dm_{RV}$ & $-$ & 0.058 & 0.817 & 0.993 & 0.990 & 0.178 & \textbf{0.000}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.822 & 0.989 & 0.989 & 0.945 & \textbf{0.000}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.188 & 0.189 & 0.181 & 0.164\\
$p$-value MCS & 0.001 & 0.004 & \textbf{0.618} & 0.000 & 0.000 & 0.003 & \textbf{1.000}\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 47.181 & 50.701 & 49.773 & 46.686 & \textbf{46.091} & 48.366 & 47.826\\
$p$-value $dm_{RV}$ & $-$ & 1 & 0 & 2 & 5 & 2 & 2\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0 & 1 & 5 & 1 & 1\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 0 & 2\\
$p$-value MCS & 26 & 25 & 26 & 23 & 26 & 25 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.161 & 0.161 & 0.264 & 0.162 & 0.162 & 0.161 & \textbf{0.152}\\
$p$-value $dm_{RV}$ & $-$ & 3 & 7 & 0 & 1 & 1 & 16\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 5 & 0 & 0 & 0 & 12\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 1 & 3\\
$p$-value MCS & 16 & 20 & 26 & 13 & 10 & 16 & 24\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h5_g3.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.344 & 0.348 & 0.335 & 0.350 & 0.349 & 0.346 & \textbf{0.331}\\
$p$-value $dm_{RV}$ & $-$ & 0.660 & 0.381 & 0.960 & 0.908 & 0.777 & 0.235\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.323 & 0.557 & 0.520 & 0.395 & 0.169\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.675 & 0.664 & 0.642 & 0.404\\
$p$-value MCS & \textbf{0.692} & \textbf{0.570} & \textbf{0.624} & \textbf{0.535} & \textbf{0.549} & \textbf{0.620} & \textbf{1.000}\\
\addlinespace[0.3em]
$QLIKE$ & 0.164 & \textbf{0.162} & 0.167 & 0.172 & 0.173 & 0.167 & 0.169\\
$p$-value $dm_{RV}$ & $-$ & \textbf{0.034} & 0.888 & 1.000 & 1.000 & 1.000 & 0.995\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.984 & 1.000 & 1.000 & 1.000 & 1.000\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.926 & 0.974 & 0.473 & 0.905\\
$p$-value MCS & 0.030 & \textbf{1.000} & \textbf{0.399} & 0.015 & 0.001 & 0.173 & 0.118\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 1.024 & 1.011 & \textbf{0.961} & 1.024 & 1.020 & 1.013 & 0.970\\
$p$-value $dm_{RV}$ & $-$ & 3 & 3 & 2 & 3 & 5 & 8\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 5 & 0 & 0 & 0 & 6\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 2 & 3\\
$p$-value MCS & 18 & 21 & 23 & 18 & 15 & 16 & 22\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.105 & 0.102 & \textbf{0.097} & 0.105 & 0.106 & 0.103 & 0.100\\
$p$-value $dm_{RV}$ & $-$ & 12 & 12 & 1 & 1 & 9 & 15\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 10 & 0 & 0 & 1 & 9\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 3 & 4\\
$p$-value MCS & 13 & 15 & 25 & 10 & 6 & 10 & 17\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h5_g4.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 0.432 & 0.432 & 0.438 & 0.425 & 0.423 & 0.425 & \textbf{0.421}\\
$p$-value $dm_{RV}$ & $-$ & 0.468 & 0.596 & 0.133 & 0.073 & \textbf{0.014} & 0.174\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.598 & 0.244 & 0.172 & 0.131 & 0.211\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0.301 & 0.259 & 0.287 & 0.102\\
$p$-value MCS & \textbf{0.810} & \textbf{0.533} & \textbf{0.848} & \textbf{0.640} & \textbf{0.875} & \textbf{0.689} & \textbf{1.000}\\
\addlinespace[0.3em]
$QLIKE$ & 0.277 & 0.273 & \textbf{0.251} & 0.283 & 0.280 & 0.275 & 0.260\\
$p$-value $dm_{RV}$ & $-$ & \textbf{0.007} & \textbf{0.000} & 0.979 & 0.861 & \textbf{0.035} & \textbf{0.000}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & \textbf{0.002} & 0.988 & 0.946 & 0.986 & \textbf{0.004}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1.000 & 1.000 & 0.999 & 0.998\\
$p$-value MCS & 0.082 & 0.104 & \textbf{1.000} & 0.069 & 0.081 & 0.044 & 0.050\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 4.503 & 4.424 & \textbf{3.793} & 4.380 & 4.431 & 4.384 & 4.099\\
$p$-value $dm_{RV}$ & $-$ & 4 & 8 & 2 & 6 & 7 & 13\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 9 & 0 & 4 & 1 & 12\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 0 & 0 & 0\\
$p$-value MCS & 10 & 17 & 26 & 10 & 13 & 14 & 24\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.176 & 0.174 & 0.182 & 0.175 & 0.171 & 0.173 & \textbf{0.160}\\
$p$-value $dm_{RV}$ & $-$ & 7 & 9 & 4 & 12 & 9 & 25\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 8 & 0 & 3 & 0 & 23\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 0 & 1 & 0 & 3\\
$p$-value MCS & 7 & 11 & 24 & 6 & 5 & 7 & 21\\
\bottomrule
\end{tabular}


==> tab_com_red/tab_com_red_h5_g5.tex <==

\begin{tabular}[t]{>{}l|cc>{}c|cccc}
\toprule
& $RV$ & $SV$ & $PV(3)$ & $SV_{bu}$ & $PV(3)_{bu}$ & $SV_{shr}$ & $PV(3)_{shr}$\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel A: DJIA index}}\\
$MSE$ & 8.894 & 9.159 & 10.340 & 8.196 & \textbf{7.929} & 8.673 & 9.186\\
$p$-value $dm_{RV}$ & $-$ & 0.786 & 0.964 & \textbf{0.017} & \textbf{0.015} & 0.170 & 0.766\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.985 & \textbf{0.031} & \textbf{0.025} & \textbf{0.020} & 0.563\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & \textbf{0.019} & \textbf{0.017} & \textbf{0.014} & \textbf{0.010}\\
$p$-value MCS & \textbf{0.332} & \textbf{0.271} & \textbf{0.492} & \textbf{0.256} & \textbf{1.000} & \textbf{0.402} & \textbf{0.310}\\
\addlinespace[0.3em]
$QLIKE$ & 4.692 & 4.691 & 4.419 & 0.241 & \textbf{0.232} & 0.247 & 0.241\\
$p$-value $dm_{RV}$ & $-$ & 0.121 & 0.381 & \textbf{0.007} & \textbf{0.007} & \textbf{0.007} & \textbf{0.007}\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 0.381 & \textbf{0.007} & \textbf{0.007} & \textbf{0.007} & \textbf{0.007}\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & \textbf{0.008} & \textbf{0.008} & \textbf{0.008} & \textbf{0.008}\\
$p$-value MCS & \textbf{0.478} & \textbf{0.481} & \textbf{0.220} & 0.176 & \textbf{1.000} & \textbf{0.481} & \textbf{0.669}\\
\midrule
\addlinespace[0.3em]
\multicolumn{8}{l}{\textit{Panel B: Individual stocks}}\\
$\overline{MSE}$ & 69.753 & 65.892 & \textbf{53.554} & 68.896 & 67.445 & 66.938 & 54.923\\
$p$-value $dm_{RV}$ & $-$ & 0 & 4 & 1 & 4 & 2 & 5\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 3 & 3 & 2 & 3 & 6\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 1 & 1 & 2 & 1\\
$p$-value MCS & 24 & 23 & 26 & 24 & 26 & 23 & 26\\
\addlinespace[0.3em]
$\overline{QLIKE}$ & 0.379 & 0.389 & 0.307 & 0.345 & 0.227 & 0.309 & \textbf{0.189}\\
$p$-value $dm_{RV}$ & $-$ & 2 & 9 & 5 & 10 & 6 & 15\\
$p$-value $dm_{SV}$ & $-$ & $-$ & 8 & 7 & 9 & 10 & 18\\
$p$-value $dm_{PV}$ & $-$ & $-$ & $-$ & 4 & 7 & 2 & 13\\
$p$-value MCS & 16 & 11 & 18 & 18 & 23 & 15 & 26\\
\bottomrule
\end{tabular}

